What's Decidable about Syntax-Guided Synthesis?

Syntax-guided synthesis (SyGuS) is a recently proposed framework for program synthesis problems. The SyGuS problem is to find an expression or program generated by a given grammar that meets a correctness specification. Correctness specifications are given as formulas in suitable logical theories, typically amongst those studied in satisfiability modulo theories (SMT). In this work, we analyze the decidability of the SyGuS problem for different classes of grammars and correctness specifications. We prove that the SyGuS problem is undecidable for the theory of equality with uninterpreted functions (EUF).We identify a fragment of EUF, which we call regular-EUF, for which the SyGuS problem is decidable. We prove that this restricted problem is EXPTIME-complete and that the sets of solution expressions are precisely the regular tree languages. For theories that admit a unique, finite domain, we give a general algorithm to solve the SyGuS problem on tree grammars. Finite-domain theories include the bit-vector theory without concatenation. We prove SyGuS undecidable for a very simple bit-vector theory with concatenation, both for context-free grammars and for tree grammars. Finally, we give some additional results for linear arithmetic and bit-vector arithmetic along with a discussion of the implication of these results.

==> EUF_is_Decidable.tex <==


\section{EUF is decidable in some cases}
This section describes an algorithm which decides the SyGuS problem for certain EUF instances, albeit in doubly-exponential time. 

Assume we are given a boolean equation $\Phi$ containing equalities between terms in the signature $\Sigma_\Phi$. 
%We will let $\Sigma_{\Phi,j}$ be the symbols in  $\Sigma_\Phi$ with rank $j$. 
Let $f$ be the function symbol appearing in $\Phi$ which is to be synthesized.
Let $G$ be a tree grammar over the alphabet $\Sigma_\Phi / \{f\} \cup \{x_1, \dots, x_k\}$, where $k$ is the rank of $f$ and the $x_i$ symbols are the variables of $f$. 
We can assume there is a deterministic bottom-up tree automaton $A_G$ such that $L(A_G) = L(G)$. 

Let $\bar{\Phi} = \bigvee_{i} \psi_i$ be $\neg \Phi$ rewritten in disjunctive normal form, where $\psi_i = \bigwedge_j \rho_{i,j}$, and $\rho_{i,j}$ is of the form $t = t'$ or $t \ne t'$ for terms $t$ and $t'$. %do we need to use the rhos? 
Our goal is find a replacement for $f$ which makes $\psi_i$ in $\bar \Phi$ unsatisfiable (or "violates $\psi_i$").  
However, a replacement which violates some $\psi_i$ might not violate another $\psi_j$. 
Therefore, to solve this problem, it is necessary to find \emph{every} replacement to $f$ which violates a $\psi_i$. 
We will show that when $\psi_i$ contains a single $f$ application,  it is possible construct an automaton $A_i$ such that $L(A_i) = L(A_G) \cap \{ e | \psi_i[f \leftarrow e]  \mbox{is UNSAT} \}$. 
We can then call the EUF solver on the new problem with replacement automaton $A_i$ and constraint formula whose negation is  $\bigvee_{j \ne i} \psi_j$ (i.e., $\psi_i$ is no longer in the negation of the constraint formula). 
This process repeats until all $\psi_i$ have been removed, at which point the problem is solvable if and only if the language of the final automaton is non-empty. 

We will now show how to solve this problem for a fixed $\psi_i$. 
Assume, without loss of generality that all $\rho_{i,j}$ in $\psi_i$ are of the form $g(c_1,\dots, c_n) = c_{n+1}$, $c_1 = c_2$, $g(c_1,\dots, c_n) \ne c_{n+1}$, or $c_1 \ne c_2$, for any $n$,  where $c_1, \dots, c_{n+1} \in \Sigma^{(0)}$ and $g \in \Sigma^{n}$ . %DO WE NEED MORE OF AN ARGUMENT AS TO WHY WE CAN DO THIS? 
Let $E_i$ be the set of $\rho$ appearing in $\Psi_i$, including the disequalities, but with all equations containing $f$ removed.
Let $E_i^+ = \{ (t,t') | t = t' \in E_i\}$ and $E_i^- = \{ (t,t') | t \ne t' \in E_i\}$.
The general idea is to create an automaton whose states represent the equivalence classes of $E_i$, then compose this automaton with $A$ to create the automaton $A_i$.

%Without loss of generality, we can assume that every $\rho$ in $\Psi_i$ is of the form $g(c_1,\dots,c_k) = c$, where $g$ is some symbol of rank $k$ and $c_1,\dots,c_k,c$ are constant symbols.

%Let $S_i = \{ s | \exists t=t' \mbox{in} \Psi_i,  s \in subterms(t) \}$.
%For each $s \in S_i$, we create a new symbol $c_s$. 
%Let $C_i = \{ c_s | s \in S_i\}$ 

Let $S$ be a set of terms. 
The \emph{subtree automaton} of $S$ is defined as \ben{cite oncina and garcia}, $SA(S) = (Sub(S), \Sigma_\Phi, \delta, Sub(S))$, with $\delta$ inductively defined as follows:
\begin{itemize}
\item $\delta(a) = c_a$, if $a \in \Sigma_{\Phi}^{(0)}$
\item $\delta(g, s_1, \dots, s_k) = s$, if $s = g(s_1, \dots, s_k)$. 
\end{itemize}
\ben{using the set of terms as the states of the above automaton is intuitive, since each term maps to it's corresponding state. But, this may be odd after we start merging states.}
%Note that for any $s \in S$, $EA^{(0)}(E_i)$ parses $s$ to the state $c_s$.
Note that $L(SA(C)) = Sub(S)$.

Given an automaton A = $(Q, \Sigma, \delta)$ and states $q,q' \in Q$, let $merge(A, q, q') = (Q / \{q'\}, \Sigma, \delta')$, where $\delta'$ is define as:
	 $\delta'(g, q_1, \dots, q_n, \{q_{n+1} \dots  q_{n+k}\}) = (g, \bar q_1, \dots, \bar q_n,  \{ \bar q_{n+1} \dots   \bar q_{n+k}\})$, where $n,k \ge 0$,  $g \in \Sigma^{(n)}$, $\bar q_i = q_i$ if $q_i \ne q'$, and $\bar q_i = q$ if $q_i = q'$.
In other words, \emph{merge} removes the state $q'$ from $A$ and changes all transitions to/from $q'$ so that they are to/from $q$.

Note that \emph{merge} can be applied to a sequence of states in any order to yield a unique automaton (up to renaming of states). Therefore, we can refer to the operation $merge(A, \{q_1, \dots, q_n\})$ in a meaningful way.

Let $S \subseteq T(\Sigma)$ and $E \subseteq T(\Sigma) \times T(\Sigma)$ such that $\{t, t' | t = t' \in E\} \subseteq S$.    The \emph{congruential tree automaton} $CTA(E, S)$ is defined as follows:
\begin{itemize} 
\item $CTA_0(E, S) = SA(S)$
\item For each $(t,t') \in E$, $CTA_{i+1}(E,S) = merge(CTA_i(E,S), t, t')$
\item While there is a $k \ge 1$ such that $(g, q_1, \dots, q_n, \{q_{n+1}, \dots, q_{n+k}\})$ is a transition in $CTA_i(E,S)$, let $CTA_{i+1}(E,S) = merge(CTA_i(E,S), \{q_{n+1}, \dots,  q_{n+k}\})$
\end{itemize}
\ben{I'm not sure whether to bother putting the above definition in pseudocode}
This process can be repeated until a fixed point is reached, which we will call $CTA(E,S)$. Note that $CTA(E,S)$ is deterministic (although possibly incomplete), $L(CTA(E,S))$ is subtree-closed, and $L(CTA(E,S))$ is the set of terms $s$ such that $CTA(E,S)[s]$ is defined . 

The following lemma can be proven by simple alterations of theorem 3.6 in $~\cite{}$ .
\ben{I'm debating whether or not to prove the whole lemma}

\begin{lemma} 
\label{parse_lemma}
Let $S \subseteq T(\Sigma)$ and $E \subseteq T(\Sigma) \times T(\Sigma)$ such that $\{t, t' | t = t' \in E\} \subseteq S$. Let $t \in L(CTA(E,S))$. Then for any other term $t' \in S$, $t \estar{E} t'$ if and only if $t' \in L(CTA(E,S))$ and $CTA(E,S)[t] = CTA(E,S)[t']$.
\end{lemma}

In particular, we consider the automaton $CTA(E^+_i,S_i)$, where $S_i = \{ s | s $ appears in $E_i$ and $s$ does not contain $f \}$. 

%We will now merge the states in $EA^{(0)}(E_i)$ according to the equalities in $E_i$, to create a sequence of automata. 
%Note, that although $EA^{(0)}(E_i)$ is deterministic, merging states can create non-determinisms, so the transition functions of $EA^{(j)}(E_i)$ maps to states.
% At step $j$ we form automaton $EA^{(j)}(E_i)$ as follows:
%\begin{itemize}
%\item If $t = t' \in E_i$, then merge states $t$ and $t'$ parse to in $EA^{(j-1)}(E_i)$
%\item If $\delta'_{E_i}(\sigma, c_{s_1}, \dots, c_{s_k}) = C$ and $|C| > 1$, then merge every state in $C$.
%\end{itemize}

%define incomplete in notation section

%With this definition of $EA(E_i)$, we can prove the following lemma.

%\begin{lemma} 
%\label{parse_lemma}
%Let $t$ be a term such that $EA(E_i)$ parses to some state $c_t$. Then for any other term $t'$, $t \leftrightarrow^*_{E_i} t'$ if and only if $EA(E_i)$ parses $t'$ to $c_t$.
%\end{lemma}
%\begin{proof}
%$\Rightarrow:$ We will prove by induction on $r$ that if $t_0 \rightarrow_{E_i} t_1 \rightarrow_{E_i} \dots t_r$ is a reduction, where $t = t_0$, then $EA(E_i)$ parses $t_r$ to $c_t$.
%The base-case where $r = 0$ clearly holds. 
%Assume the property holds for all derivations of length less than or equal to $r$. Let $t_{r+1}$ be a term such that $t_r \rightarrow_{E_i} t_{r+1}$. In other words, there is an equation $s = s'$ in $E_i$ such that $s$ occurs in $t_r$ and replacing $s$ with $s'$ in $t_r$ yields $t_{r+1}$. By the construction of $EA(E_i)$, $s$ and $s'$ must parse to the same state. Therefore, $t_r$ and $t_{r+1}$ must parse to the same state.
%$\Leftarrow:$:  \ben{I'm holding off on writing this part, since I think I have a simpler proof, but I want to check it first.} 
%\end{proof}


Now that we have seen how to construct the automaton $CTA(E^+_i,S_i)$, we need to show how to compose it with the given automaton $A_G$ of possible replacements to $f$.
Note that if there is a $t \ne t' \in E_i^-$ such that $CTA(E^+_i,S_i)$ parses $t$ and $t'$ to the same state, then $\Psi_i$ is inconsistent for any $f$ substitution.
So we will assume that this isn't the case. 
Assume, that there is a single equation $f(s_1, \dots, s_k) = s'$ containing $f$ in $\Psi_i$.
Replacing $f$ with $e$ in $\Psi_i$ is equivalent to replacing the equation $f(s_1, \dots, s_k) = s'$ with $e[x_1 \leftarrow s_1, \dots, x_k \leftarrow s_k] = s'$.
Let $e' = e[x_1 \leftarrow s_1, \dots, x_k \leftarrow s_k]$.
The congruential tree automata after replacing $f$ with $e'$ in $\Psi_i$ then becomes $CTA(E^+_i \cup \{e' = s'\} ,S_i \cup \{e'\}) $
We will show that our choice of $e$ can only yield a contradiction when $e' \in L( CTA(E^+_i,S_i))$.% the automaton $CTA(E^+_i \cup \{e' = s'\} ,S_i  \cup \{e'\})$ parses two terms $t$ and $t'$ to the same state when $t \ne t' \in E_i$. 


 

\begin{lemma}
If $e' \not\in CTA(E^+_i,S_i)$, then $\Psi_i[f \leftarrow e]$ is consistent. 
\end{lemma}
\begin{proof}
Let $t \ne t' \in E_i^-$, let $CTA(E^+_i,S_i)[t] = q$ and  $CTA(E^+_i,S_i)[t] = q'$. 
We know that $q$ and $q'$ are defined by the definition of $S_i$, and we have already assumed that $q \ne q'$.
Assume $e' \not\in L(CTA(E^+_i,S_i))$.
Then the state $CTA(E^+_i,S_i \cup \{e'\})[e'] = \bar q$ is not in $CTA(E^+_i,S_i)$. 
Any outgoing transitions from $\bar q$ in $CTA(E^+_i,S_i \cup \{e'\})$ must lead to an accepting state, since all states in $CTA(E^+_i,S_i \cup \{e'\})$ are accepting.
Since $L(CTA(E^+_i,S_i))$ is subtree-closed, this would imply that $e' \in L(CTA(E^+_i,S_i))$ . 
Therefore, $\bar q$ cannot have any outgoing transitions.
By the definition of CTA, this implies that $CTA(E^+_i \cup \{e' = s'\} ,S_i \cup \{e'\}) = merge(CTA(E^+_i, S_i \cup \{e'\}), e', s')$
%But each of these new states has exactly one outgoing transition and so can't induce a merging of states as described in the second bullet of the construction of $EA(E_i)$. \ben{I'm going to try to figure out notation to use to make this statement less odd}


%So any two distinct states in $EA(E_i)$ must remain distinct in $EA(E_i\cup \{e' = s'\})$.


So $CTA(E^+_i \cup \{e' = s'\} ,S_i \cup \{e'\})[t] = merge(CTA(E^+_i, S_i \cup \{e'\}), e', s')[t] = q \ne q' = merge(CTA(E^+_i, S_i \cup \{e'\}), e', s')[t'] = CTA(E^+_i \cup \{e' = s'\} ,S_i \cup \{e'\})[t']$
Therefore $\Psi_i[f \leftarrow e]$ is consistent.
\end{proof}

By the above lemma, we can restrict ourselves to considering expressions $e \in L(CTA(E^+_i,S_i))$.
Let $CTA(E^+_i,S_i)[s'] = q_{s'}$
For any state $q$ in $CTA(E^+_i,S_i)$, we can find an $s$ such that $CTA(E^+_i,S_i)[s] = q$  check if $CTA(E^+_i \cup {s = s'}, S_i)$ yields a contradiction.
Let $\bar Q$ be the set of states which yield such a contradiction.
Using a very similar construction to the product of two automata, we can create the automaton $A_i$ we described at the beginning of this section.

Let $A_i = (Q \times \bar Q, \Sigma \cup \{x_1, \dots, x_k\} , \delta_i, F \times \bar Q)$, such that:
\begin{itemize}
\item $\delta_i(x_j) = (\delta(x_j), c_{s_j})$
\item $\delta_i(g, (q_1,\bar q_1), \dots, (q_r,\bar q_r)) = (\delta(g, q_1, \dots, q_r), \delta'(\bar q_1, \dots, \bar q_r))$, where $\delta'$ is the transition function for $CTA(E^+_i,S_i)$.
\end{itemize}

It is easy to check that the trees yielded by $A_i$ are precisely the trees which yield contradictions when substituted for $f$.

\ben{there is a bug when considering multiple f instances in a conjunction}









==> euf.tex <==

This section proves that the SyGuS problem for uninterpreted functions with equality (EUF) is undecidable. Our proof is based on a reduction from the Post correspondence problem (PCP)~\cite{post1946variant}. 
The reduction relies on a tree grammar that produces only applications of unary function symbols, showing that for EUF, even basic instances of SyGuS are undecidable. 
%In particular, the constructed problem requires the synthesis of a single function and only contains functions of arity 1. 


%The proof is a reduction from the Post correspondence problem (PCP)~\cite{post1946variant}.
Recall that the Post correspondence problem is to decide, given pairs of finite strings $(s_1, s_1'), (s_2, s_2'),\ldots,(s_n,s'_n)$, the existence of a non-empty sequence of integers $i_1,i_2,\dots,i_k$ ($1\leq i_j \leq n$ for all $j$) such that $s_{i_1}s_{i_2}\dots s_{i_k} = s'_{i_1}s'_{i_2}\dots s'_{i_k}$. 
PCP is undecidable even when the strings only contain two symbols, so we will focus on PCP problems with the alphabet $\{a,b\}$. 

As an example consider the Post correspondence problem for the pairs of strings $(s_1, s_1') = (bb,b)$, $(s_2, s_2') = (ab,ba)$, and  $(s_3, s_3') = (b,bb)$. 
The sequence of indices 1 2 2 3 is a solution: $s_1s_2s_2s_3 = bbababb = s'_1s'_2s'_2s'_3$. 


\begin{theorem}
\label{thm:euf_und}
SyGuS for EUF is undecidable for the class of EUF-compatible tree grammars. 
%problems containing at least 5 uninterpreted functions (all of which have arity 1) and a single replacement tree grammar. \ben{It's very weird having to write a complete sentence whenever we need to describe a SyGuS problem. Can we define a problem as a tuple, such as $(\varphi, f, G)$ ?}
\end{theorem}

\begin{proof}
Let $P = (s_1,s'_1), (s_2,s_2'),\dots,(s_n,s'_n)$ be an instance of PCP and let $g_a$, $g_b$, $g'_a$, $g'_b$, and $h$ be (distinct) unary function symbols. 
From the PCP instance, we will construct an EUF-compatible tree grammar $G_P=(N,S,T,R)$ and a correctness constraint $\varphi_P$. %, such that a solution to the given correspondence problem will exist if, and only if, $G_P$ generates an expression $e$ such that $\varphi[f/e]$ is valid in all models of $\Sigma$.

%\ben{Should we use a constant c as the argument to the grammar, or a variable, x. The SyGuS paper seems to argue that we use x. (such as the max(x,y) example).}

The terminals of the grammar are ``$x$'', ``$g_a$'', ``$g_b$'', ``$g_a'$'', ``$g_a'$'', ``$h$'', ``$($'', and ``$)$''.
Given a pair $(s_j, s_j')$ with $|\sigma|=r$ and $|\sigma'| = r'$, we add the following production rules to $R$:
\[p^S_j = S \rightarrow g_{s_j(1)}(g_{s_j(2)}(\dots(g_{s_j(r)}(g'_{s_j'(1)}(g'_{s_j'(2)}(\dots(g'_{s_j'(r')}(V))\dots))))\dots)) \ \]
\[p^V_j = V \rightarrow g_{s_j(1)}(g_{s_j(2)}(\dots(g_{s_j(r)}(g'_{s_j'(1)}(g'_{s_j'(2)}(\dots(g'_{s_j'(r')}(V))\dots))))\dots)) \,,\]
where $s_j(i)$ is the $i$-th symbol in the string $s_j$.
(The production rules occur twice in similar form, once for the start symbol $S$ and once for $V$, to guarantee that at least one pair of symbols $(s_j,s_j')$ is produced and so the corresponding PCP solution is non-empty.)
To allow the termination of a production sequence we further add the production $p_{end} = V \rightarrow x$.

Intuitively, for any sequence of integers $i_1,i_2,\dots,i_k$ such that $s_{i_1}s_{i_2}\dots s_{i_k} = s'_{i_1}s'_{i_2}\dots s'_{i_k}$, we would like $\varphi$ to be satisfied by the string constructed by following the productions $p^S_{i_1}, p^V_{i_2},\dots,p^V_{i_k},p_{end}$.
(Since there is at most one non-terminal on the right-hand side of each production rule, this description yields a unique expression.)
We now construct the correctness constraint $\varphi$ such that chains of productions are valid iff the corresponding sequence of indices is a solution to the PCP instance.

Let $\psi$ be the conjunction of the following constraints:
\[
\begin{array}{rcl}
g_{a}(g'_{b}(y)) &=& g'_{b}(g_{a}(y)) \\
g_{b}(g'_{a}(y)) &=& g'_{a}(g_{b}(y)) \\
h(g_a(g'_a(y))) &=& h(y) \\
h(g_b(g'_b(y))) &=& h(y)
\end{array}
\]

That is, we require that applications of the functions $g_a,g_b$ commute with applications of the functions $g'_a,g'_b$ (but not necessarily $g_a$ with $g_b$ or $g'_a$ with~$g'_b$). 
Further, applications of $g_a$ and $g'_a$ and likewise of $g_b$ and $g'_b$ are required to cancel each other when they occur directly inside an application of $h$. 
We then define the correctness constraint $\varphi_P$ to be $\psi \rightarrow h(f) = h(x)$. 
Note that $\varphi$ is constructed independently of the PCP instance being studied. 

%The antecedent $\psi$ is constructed so that the $g$ function applications \emph{commute} with the $g'$ applications. However, the $g_a$ applications do not necessarily commute with the $g_b$ applications (similar for $g'_a$ and $g'_b$). 
%We formalize these notions through the functions $str$ and $str'$, which map $L(G_P)$ to $\{a,b\}^*$. 
%We will only show the definition of $str$, as $str'$ is defined analogously. 
%Here, $s$ is some string of $g$ and $g'$ function applications on some variable $x$ and $\sigma \in T$:
%\begin{align*}
%str(h(s)) &= str(s) \\
%str(g_\sigma(s)) &= \sigma \cdot str(s) \\
%str(g'_\sigma(s)) &= str(s) \\
%str(x) &= \lambda
%\end{align*}
%
%With these definitions, we can prove the first lemma of this section. 

The easy direction is to show that every sequence of indices $i_1,i_2,\dots,i_k$ such that $s_{i_1}s_{i_2}\dots s_{i_k} = s'_{i_1}s'_{i_2}\dots s'_{i_k}$ gives us a sequence of productions $p^S_{i_1}, p^V_{i_2},\dots,p^V_{i_k},\linebreak p_{end}$ that produces an expression that is valid under every model $M$.
Given any model $M$ that satisfies the antecedent $\psi$, we can commute the outermost applications of a primed and an unprimed function (of $g_a$, $g_b$, $g_a'$, and $g_b'$) to the ``top''. 
By repeatedly pulling matching applications to the top and eliminating them inside the application of $h$, we arrive at the term $h(x)$, which satisfies the correctness specification.
%
%%\begin{lemma}
%%Let $P = (s_1,s'_1), (s_2,s_2'),\dots,(s_n,s'_n)$ be a PCP instance.
%%If $P$ has a solution, then there is some $e \in L(G_P)$ such that for all models $M$ of EUF it holds $M \models \varphi_P[f\backslash e]$. 
%%\end{lemma}
%
%\begin{proof}
%Let $i_1,i_2,\dots,i_k$ be a sequence of integers such that $s_{i_1}s_{i_2}\dots s_{i_k} = s'_{i_1}s'_{i_2}\dots s'_{i_k}$. 
%Let $e$ be the string derived in $G_P$ by the production applications $p^S_{i_1}, p^V_{i_2},\dots,p^V_{i_k},p_{end}$.
%We can see that $str(e) =  s_{i_1}s_{i_2}\dots s_{i_k} = s'_{i_1}s'_{i_2}\dots s'_{i_k} = str'(e)$. Therefore, we can write $e = h(g_{\sigma_1}(\dots (g_{\sigma_i}(g'_{\sigma_1}(\dots g'_{\sigma_r}(x)\dots ))\dots )))$, where $g_{\sigma_j}$ and $g'_{\sigma_j}$ are the $j^{th}$ instances of a $g$ and $g'$ application in $e$, respectively. Let $M$ be some model. If $M \not \models \forall y \psi$, then $M \models \varphi$ trivially. Assume $M \models \forall y \psi$. Then, when interpreted in $M$ with $x$ equal to any $c \in \text{dom}(M)$, $e =  h(g_{\sigma_1}(g_{\sigma_2}(\dots g_{\sigma_i}(g'_{\sigma_1}(\dots g'_{\sigma_r}(c)))))) = h(g_{\sigma_1}(g'_{\sigma_1}(g_{\sigma_2}(\dots g_{\sigma_i}(\dots (g'_{\sigma_r}(c))\dots )\dots )))) = h(g_{\sigma_2}(\dots g_{\sigma_i}(\dots (g'_{\sigma_r}(c))\dots )\dots ))$. \ben{This description feels a bit awkward. Does anyone have any suggestions how to improve it?}  So, by an inductive argument, we can move each successive $g'_i$ towards the outside of $e$ to get $h(g_{\sigma_1}(g'_{\sigma_1}(s))) = h(s)$, where $s$ is the remaining set of function applications in $e$. We can repeat this process until we get $e = h(c)$. Therefore, $M \models \forall x(e = h(x))$, so $M \models \varphi[f / e]$. 
%\qed
%\end{proof}
%Let $G = (N,T', P, S)$, where $N$ is a set of non-terminals, $T'$ is a set of terminals, $P$ is a set of production rules, and $S$ is a starting non-terminal. Let $T' $ contain the symbols $c, h, g_{a}, g'_{a}, g_{b}$, and  $g'_{b}$, as well as '(' and ')' and ',' . Let $N = \{ S, A \}$.
%Add the productions  and $p_{end} = A \rightarrow c$ to $P$.



%\begin{example}
%\label{exmp:pcp_grammar}
%Let $T = \{a,b\}$, $(s_1,s_1') = (bb,b)$, and $(s_2,s_2') = (a,ba)$. The string $s_1s_2 = bba = s_1's_2'$ is a solution to the Post correspondence problem. The corresponding SyGuS grammar would have production rules:
%\begin{align*}
%p_{start} = S &\rightarrow h(S')\\
%p_{end} = A &\rightarrow x \\
%p'_1 = S' &\rightarrow g_b(g_b(g_b'(A)))\\
%p'_2 = S' &\rightarrow g_a(g_b'(g_a'(A)))\\
%p_1 = A &\rightarrow g_b(g_b(g_b'(A)))\\
%p_2 = A &\rightarrow g_a(g_b'(g_a'(A)))\\
%\end{align*}
%
%
%A SyGuS solver might apply the productions $p_{start},p'_1,p_2,p_{end}$ to derive the expression $e = h(g_b(g_b(g_b'(g_a(g_b'(g_a'(c)))))))$. We can see that $str(e) = bba = str'(e)$. For any EUF model $M$ such that $M \models \forall y \psi$ and $x=c$ for any $c \in \text{dom}(M)$,  we can see that the following equivalences hold in $M$:
%\begin{align*}
%e &= h(g_b(g_b(g_b'(g_a(g_b'(g_a'(c)))))))\\
%&= h(g_b(g'_b(g_b(g_a(g_b'(g_a'(c)))))))\\
%&= h(g_b(g_a(g_b'(g_a'(c)))))\\
%&= h(g_b(g'_b(g_a(g_a'(c)))))\\
%&= h(g_a(g_a'(c)))\\
%&= h(c)
%\end{align*}
%
%Therefore $M \models \forall x (e = h(x))$, so $M \models \varphi[f / e]$. 
%\qed
%\end{example}

We now turn to the other direction. 
Let $i_1,i_2,\dots,i_k$ be a sequence of indices that is not a solution to the PCP problem. 
We show that for the expression obtained by the productions $p^S_{i_1}, p^V_{i_2},\dots,p^V_{i_k}, p_{end}$ there is a model that invalidates the correctness specification $\varphi_P[f / e]$. 
%
%\begin{lemma}
%Let $P = (s_1,s'_1), (s_2,s_2'),\dots ,(s_n,s'_n)$ be a PCP instance, for  $T = \{a,b\}$ and $s,s' \in T^*$. If P has no solution, then there is no solution to the SyGuS problem to synthesize $f$ from grammar $G_P$ satisfying constraints $\varphi$. 
%\end{lemma}
%
%\begin{proof}
We construct $M$ such that the antecedent $\psi$ holds for all $y$, but $M$ does not model $h(e) = h(x)$ for any $e \in L(G_P)$. 
We define $\text{dom}(M) = \{a,b\}^* \times \{a,b\}^*$ and define $g_a$, $g'_a$, $g_b$, and $g'_b$ to be functions from  $\text{dom}(M)$ to $\text{dom}(M)$. 
We define these functions as follows, for $\alpha,\beta \in \{a,b\}$ and $s,s' \in \{a,b\}^*$:
\begin{align*}
g_\alpha((s,s')) &= (\alpha s, s')\\
g'_\alpha((s,s')) &= (s, \alpha s') \\
h((\alpha s, \beta s')) &= h((s,s')) \text{, if } \alpha = \beta\\
h((\alpha s, \beta s')) &= (\alpha s, \beta s') \text{, if } \alpha \neq \beta
\end{align*}

That is, $g_a$ and $g_b$ add elements to the first list, $g_a'$ and $g_b'$ add elements to the second list, and $h$ removes the common prefix. 
It is easy to verify that these function definitions satisfy the antecedent $\psi$.

Assume the variable $x$ in the correctness specifications is instantiated with the tuple $(\varepsilon,\varepsilon)$ of empty strings. 
If the sequence of letters of $a$ and $b$ produced by the sequence of indices is different in length (say the first is shorter), then we can apply the function definitions above such that the correctness constraint reduces to $(\varepsilon,s)=(\varepsilon,\varepsilon)$ with $s\neq \varepsilon$ and is thus violated. 
If the sequences of letters $a$ and $b$ are of the same length but have a position in which they are different, we can apply the rules above to eliminate the common prefix and again arrive at a tuple that is different to $(\varepsilon,\varepsilon)$.

We conclude that for any given sequence of indices that is not a solution to $P$, the corresponding production does not yield an expression that is valid for every model. 
Since any sequence of productions of the grammar corresponds also to a sequence of indices this concludes the proof. 
%We can see that $M \models \forall y \psi$. To see that $M \not \models \forall x (e = h(x))$, let $e \in L(G_P)$ be generated by the productions rules $p_{start},p_{i_1},p_{i_2},\dots ,p_{i_k},p_{end}$.  Write $e = h(g''_{\sigma_1}(g''_{\sigma_2}(\dots (g''_{\sigma_n}(x)) \dots )))$, where $\sigma_i \in T$ and $g''_{\sigma_i}$ equals $g_{\sigma_i}$ or $g'_{\sigma_i}$. We can check from the definition of $M$ that $M \models g''_{\sigma_1}(g''_{\sigma_2}(\dots (g''_{\sigma_n}(s)) \dots )) = (str(e),str'(e),s)$ for any string $s$. Since $P$ has no solution, we know that $s_{i_1}s_{i_2}\dots s_{i_k} \ne s'_{i_1}s'_{i_2}\dots s'_{i_k}$, so $str(e) \ne str'(e)$. Because $M \models \forall x (e = h((str(e),str'(e),x)))$, this implies that $M \models \forall x(e = \lambda)$. Therefore, there is no $e \in L(G_P)$ such that $M \models \forall x (e = h(x))$, so the SyGuS problem does not have a solution.
%\qed
%\end{proof}
\qed
\end{proof}



%\begin{example}
%\label{exmp:pcp_grammar}
%The correspondence problem from example \ref{exmp:pcp} would yield the following grammar. 
%\begin{align*}
%S \rightarrow & h(A) \\
%A \rightarrow & g_b(g_b(g'_b(A))) \ |  \\
%              & g_a(g_b(g_b'(g_a'(A)))) \ | \\
%              & g_b(g_b'(g_b'(A))) \ | \\
%              c
%\end{align*}
%The solution to the correspondence problem shown in \ref{exmp:pcp} corresponds to the expression derived by $S \Rightarrow h(A) \Rightarrow h(g_b(g_b(g'_b(A)))) \Rightarrow h(g_b(g_b(g'_b(g_a(g_b(g'_b(g'_a(A)))))))) \Rightarrow h(g_b(g_b(g'_b(g_a(g_b(g'_b(g'_a(THIS IS TOO LOGN))))))))
%\end{example}

\subsection{Implications for Arrays}


\begin{corollary}
     SyGuS for AR is undecidable with the class of AR-compatible tree grammars, even when arrays cannot be nested. 
    \label{cor:arr_und}
\end{corollary}
\begin{proof}
We can recast the functions in the proof of Theorem \ref{thm:euf_und} as arrays to create a SyGuS problem in AR, which can only be solved if there exists a solution to the original SyGuS problem in EUF.
Take any Post-correspondence problem $P$ and grammar $G_P$ as defined above.
Let $\varphi$ be the EUF constraint formula defined above. 
We can replace any function call $g(a)$ in $\varphi$ or $G_P$ with the statement $\text{read}(g,a)$ to get a SyGuS problem in AR.
It is easy to check that this problem can be solved if, and only if, the original SyGuS problem in EUF is solvable.
\qed
\end{proof}

\subsection{Extending the Undecidability Result to Regular Grammars}

In the proof of Theorem~\ref{thm:euf_und}, we assumed that the provided grammar was a tree grammar with at most one non-terminal on the right side of any production rule. 
We may wonder whether an even more restricted grammar could allow the SyGuS problem to become decidable. Consider the right-regular grammars, which generate the regular languages. 
These grammars cannot even produce the language of well-matched parenthesis, so we cannot expect them to only yield well-formed strings, that is strings that are expressions in the theory. 
However, given a right-regular grammar $G_{reg}$ and the grammar of well-formed strings $U$, we can construct a context-free grammar $G'$ such that $L(G') = L(G_{reg}) \cap L(U)$. 
%See that $G'$ generates precisely the set of well-formed strings generated by $G_{reg}$. 
Unfortunately, even in this restricted form, we can still specify the grammars used in the above undecidability proofs of EUF and arrays.

\begin{corollary}
SyGuS for EUF with right-regular grammars is undecidable.
\end{corollary}
\begin{proof}
%We reduce to PCP.
Let $P = (s_1,s'_1), (s_2,s_2'),\dots,(s_n,s'_n)$ be a PCP instance. 
We construct $G_{reg}$ with the following productions:
\begin{align*}
S &\rightarrow \quad xV \\
V &\rightarrow \quad )V \quad | \quad )
\end{align*}

For each $(s_i, s'_i)$ in $P$, with $|s_i|=r$ and $|s_j'|=r'$, we add the following two production rules to $G_{reg}$:
\[
S\rightarrow \quad g_{s_j(1)}(g_{s_j(2)}(\dots(g_{s_j(r)}(g'_{s_j'(1)}(g'_{s_j'(2)}(\dots(g'_{s_j'(r')}(\ V
\]
\[
V\rightarrow \quad g_{s_j(1)}(g_{s_j(2)}(\dots(g_{s_j(r)}(g'_{s_j'(1)}(g'_{s_j'(2)}(\dots(g'_{s_j'(r')}(\ V
\]
%\[V \rightarrow g_{\sigma_1}(g_{\sigma_2}(\dots (g_{\sigma_k}(g'_{\sigma'_1}(g'_{\sigma'_2}(\dots (g'_{\sigma'_r}(A\]

We can see that the set of well-formed expressions from $G_{reg}$ precisely matches those of grammar $G_P$ as defined in Theorem~\ref{thm:euf_und}. \qed
\end{proof}

%Therefore, the SyGuS problem remains undecidable, even when right-regular grammars are provided.


\begin{corollary}
    SyGuS for AR is undecidable with regular languages, even when arrays cannot be nested.
\end{corollary}
\begin{proof}
%We reduce to PCP. 
Let $P = (s_1,s'_1), (s_2,s_2'),\dots ,(s_n,s'_n)$ be a PCP instance. We create a grammar $G_{reg}$ and add the following productions:
\begin{align*}
S &\rightarrow \quad xV \\
V &\rightarrow \quad )V \quad | \quad )
\end{align*}

\renewcommand{\read}[0]{\mathit{read}}

For each $(s_i, s'_i)$ in $P$, with $|s_i|=r$ and $|s_j'|=r'$, we add the following transitions to $G_{reg}$: 
\[
\begin{array}{rl}
S\rightarrow  \quad 
& \read(g_{s_j(1)},\read (g_{s_j(2)}, \dots, \read(g_{s_j(r)}, \\ 
& \qquad \read(g'_{s_j'(1)},\read(g'_{s_j'(2)},\dots,\read(g'_{s_j'(r')},\ V \\
V\rightarrow  \quad 
& \read(g_{s_j(1)},\read (g_{s_j(2)}, \dots, \read(g_{s_j(r)}, \\ 
& \qquad \read(g'_{s_j'(1)},\read(g'_{s_j'(2)},\dots,\read(g'_{s_j'(r')},\ V 
\end{array}
\]
%\[V \rightarrow read(g_{\sigma_1}, read(g_{\sigma_2}, \dots read(g_{\sigma_k}, read(g'_{\sigma'_1}, read(g'_{\sigma'_2}, \dotsread(g'_{\sigma'_r},A\]

The well-formed expressions of $G_{reg}$ precisely match the expressions from Corollary~\ref{cor:arr_und}. 
%And so by using the same constraints for corollary \ref{cor:arr_und}, we can see that the SyGuS problem has a solution if and only if $P$ has a solution. 
\qed
\end{proof}




\subsection{On Well-Formed and Ill-Formed Expressions}

When we allow the grammar in a SyGuS problem to produce ill-formed expressions and consider the intersection with the expressions of the background theory, as in the previous subsection, we can derive a very strong proof of undecidability. 
The proof only relies on the well-formedness of expressions, and holds independently of the interpretation of the function symbols.
That is, the proof also holds for theories other than EUF. 
%The standard formulation of SyGuS implicitly assumes that the grammars only produce well-formed expressions. 
%We can extend the problem definition of SyGuS to grammars that potentially produce ill-formed expressions by considering its intersection with the grammar of the background theory. 
%In the following we show that this definition leads to a very strong proof of undecidability, which depends, however, on the syntax of background theories. 


\begin{theorem}
SyGuS for CFGs is undecidable for any theory $\mathcal{T}$ with domain $D$ containing 
two function symbols $f:D^m\to D$ and $g:D^n\to D$ of different non-zero arities $(m\neq n$ and $m,n>0)$. 
\end{theorem}

\begin{proof}
This proof is by reduction from the Post-correspondence problem.
Let $h$ and $g$ be function symbols in $sig(\mathcal T)$ of arity $m$ and $n$, respectively, where $m \ne n$ and $m,n>0$.
Let $P = (s_1,s'_1), (s_2,s_2'),\dots,(s_k,s_k')$ be a PCP instance with alphabet $\{a,b\}$. 
We construct a grammar $G_P = (N,S,T,R)$ so that sequences of indices that are a solution to the PCP problem correspond to derivations in the grammar that produce a well-formed expression, and where sequences of indices that are not a solution to the PCP problem correspond to derivations in the grammar that produce an ill-formed expression. 

For each pair $(s_i,s_i')$ in $P$ we construct two terminals $\sigma_i$ and $\sigma_i'$ in $T$. 
For each position $j$ in the sequence $s_i\in\{a,b\}^*$ we define $\sigma_i(j)=``f("$ if $s_i(j)=a$ and $\sigma_i(j)=``g("$ if $s_i(j)=b$. 
Correspondingly, we define for each position $j$ in $s_i'\in\{a,b\}^*$ that 
\[
\sigma_i'(r+1-j)=\left(``,x"\right)^{m-1} + ``)" \quad\text{if }  s_i'(j)=a \quad\text{ and } 
\]
\[
\sigma_i'(r+1-j)=\left(``,x"\right)^{n-1} + ``)"  \quad\text{if }  s_i'(j)=b \,, \qquad\quad
\]
where $r=|s_i'|$ is the length of the word $s_i'$ and $x$ is some variable.
That is, the terminals $\sigma_i'$ are lists of lists of arguments of length $m-1$ and $n-1$ that are supposed to match the function calls of $f$ and $g$, respectively. 
We are only providing $m-1$ and $n-1$ arguments, respectively, as the first argument will (except for the innermost level) be the next function call.
Within the terminals $\sigma_i'$ the argument lists occur in \emph{reverse order} compared to the strings~$s_i'$. 

We add two nonterminals $S$ and $V$ and for each pair of strings $(s_i,s_i')$ in $P$ we add one production rule for both nonterminals:
\[
S \rightarrow \sigma_i V \sigma'_i \quad\text{and}\quad V \rightarrow \sigma_i V \sigma'_i
\]
That is, the production rules produce a string over opening parts of function calls ($\sigma_i$) matching, in reverse order, a string of argument lists ($\sigma_i'$) which each are reversed internally. 
Finally, we add one production rule $V\rightarrow ``x"$, which provides the ``missing'' argument for the innermost function call. 
(The need for two nonterminals comes from the fact that we have to disallow the derivation yielding only $x$.)

We can then define the correctness constraint $\varphi$ as $f = f$, where $f$ must be replaced by some expression in $G_P$. 
For this correctness constraint, each syntactically correct replacement of $f$ is valid in every theory. 
Thus, this SyGuS problem has a solution, if and only if the PCP instance $P$ has a solution. 
\qed
\end{proof}

\begin{example}
Let $(s_1,s'_1)=(bb,b)$, and $(s_2,s'_2) = (a,ba)$. Then $s_1s_2 = bba = s'_1s'_2$ is a solution to the Post-correspondence problem. Let $f$ and $g$ be functions in the background theory $\mathcal{T}$ with arities 1 and 2, respectively. We can associate $f$ with $a$ and $g$ with $b$. 
The grammar $G_P$ can produce the expression $g(g(f(x),x),x)$, which corresponds to the solution \emph{bba}. 
\end{example}




